Understanding the Benefits of Hardware-Accelerated Communication in Model-Serving Applications

It is commonly assumed that the end-to-end networking performance of edge offloading is purely dictated by that of the network connectivity between end devices and edge computing facilities, where ongoing innovation in 5G/6G networking can help. However, with the growing complexity of edge-offloaded computation and dynamic load balancing requirements, an offloaded task often goes through a multi-stage pipeline that spans across multiple compute nodes and proxies interconnected via a dedicated network fabric within a given edge computing facility. As the latest hardware-accelerated transport technologies such as RDMA and GPUDirect RDMA are adopted to build such network fabric, there is a need for good understanding of the full potential of these technologies in the context of computation offload and the effect of different factors such as GPU scheduling and characteristics of computation on the net performance gain achievable by these technologies. This paper unveils detailed insights into the latency overhead in typical machine learning (ML)-based computation pipelines and analyzes the potential benefits of adopting hardware-accelerated communication. To this end, we build a model-serving framework that supports various communication mechanisms. Using the framework, we identify performance bottlenecks in state-of-the-art model-serving pipelines and show how hardware-accelerated communication can alleviate them. For example, we show that GPUDirect RDMA can save 15--50\% of model-serving latency, which amounts to 70--160 ms.

==> figures-latex/multi_b2b_mat_overhead_deeplabv3.tex <==
\begin{figure*}
\centering
    \begin{subfigure}{0.32\textwidth}
       	\centering
	   \includegraphics[width=\textwidth]{figures/multiple_b2b_overhead_deeplabv3-CLASSIFICATION_MAT-ZMQ.png}
	   \caption{ZMQ}%
\label{fig:multiple_b2b_mat_deeplabv3_overhead_zmq}
    \end{subfigure}
\hfill
    \begin{subfigure}{0.32\textwidth}
       	\centering
	   \includegraphics[width=\textwidth]{figures/multiple_b2b_overhead_deeplabv3-CLASSIFICATION_MAT-GPU-HOST_ADDRESSING.png}
	   \caption{RDMA}%
	   \label{fig:multiple_b2b_mat_deeplabv3_overhead_rdma}
    \end{subfigure}
\hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/multiple_b2b_overhead_deeplabv3-CLASSIFICATION_MAT-GPU-CUDA_ADDRESSING.png}
        \caption{GDR}%
    \label{fig:multiple_b2b_mat_deeplabv3_overhead_gpudirect}
    \end{subfigure}
\caption{Overhead Breakdown across steps when serving Raw Images using \texttt{DeepLabv3}}%
\label{fig:multiple_b2b_mat_deeplabv3_overhead}
\end{figure*}


==> tables/metrics.tex <==
\begin{table}[t]
\centering
\caption{Performance Metrics}
\label{tab:metrics}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{||c|c||}
    \hline \hline
    \textbf{Metric} & \textbf{Description}\\ \hline \hline \hline
    \texttt{Total Time} & Total latency witnessed by the client. \\
    \texttt{Request Time} & Time used to send the request. \\
    \texttt{Copy Time} & H2D copy time + D2H copy Time. \\
    \texttt{Preprocessing Time} & Time used in preprocessing. \\
    \texttt{Inference Time} & Time used in DNN processing (inference). \\
    \texttt{Response Time} & Time used to send the response.\\
    \texttt{CPU Time} & CPU Time (user and kernel time).\\
    \texttt{Memory Usage} & RAM and GPU Memory usage.\\    
    \hline \hline
\end{tabular}%
}
\end{table}


==> tables/models.tex <==
\begin{table}[t]
\centering
\caption{DNN Models}
\label{tab:models}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{||c|c|c|c|c||}
\hline \hline
 \textbf{Model} & \textbf{Task}  & \textbf{Dataset} & \textbf{Model Size} & \textbf{IO Size} \\ \hline \hline \hline
  \texttt{MobileNetV3} & Classification & ImageNet\cite{imagenet}  & Small & Small\\
 \texttt{ResNet50} & Classification & ImageNet \cite{imagenet} & Medium & Small\\
  \texttt{EfficientNetB0} & Classification & ImageNet\cite{imagenet}  & Medium & Small\\
 \texttt{WideResNet101} & Classification & ImageNet\cite{imagenet}  & Large & Small\\
  \texttt{YoloV4} & Detection & COCO\cite{coco} & Large & Medium   \\
 \texttt{DeepLabV3\_ResNet50} & Segmentation & COCO\cite{coco} & Large & Large  \\
 \hline \hline
\end{tabular}%
}
\end{table}

==> tables/models_old.tex <==
\begin{table}[t]
\centering
\caption{DNN Models}
\label{tab:models}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{||c|c|c|c|c||}
\hline \hline
 \textbf{Model} & \textbf{Task}  & \textbf{Dataset} & \textbf{Input Shape} & \textbf{Output Shape} \\ \hline \hline \hline
 \texttt{ResNet50} & Classification & ImageNet \cite{imagenet} & 3$\times$224$\times$224 & 1$\times$1000\\
 \texttt{WideResNet101} & Classification & ImageNet\cite{imagenet}  & 3$\times$224$\times$224 & 1$\times$1000\\
  \texttt{MobileNetV3} & Classification & ImageNet\cite{imagenet}  & 3$\times$224$\times$224 & 1$\times$1000\\
  \texttt{EfficientNetB0} & Classification & ImageNet\cite{imagenet}  & 3$\times$224$\times$224 & 1$\times$1000\\
 \texttt{DeepLabV3\_ResNet50} & Segmentation & COCO\cite{coco} & 3$\times$520$\times$520 & 2$\times$21$\times$520$\times$520  \\
  \texttt{YoloV4} & Detection & COCO\cite{coco} & 3$\times$416$\times$416 & \begin{tabular}{@{}c@{}}S$\times$S$\times$3$\times$85, \\ S = $\{13, 26, 52\}$\end{tabular}   \\
 \hline \hline
\end{tabular}%
}
\end{table}
\writingtodo{add size and summarize dataset. comp/communication heavy.}

==> tables/servers.tex <==

\begin{table}[t]
\centering
\caption{Servers}
\label{tab:server}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{||c|c|c|c|c||}
\hline \hline
 \textbf{Server}& \textbf{Server Type} & \textbf{CPU} & \textbf{GPU} & \textbf{NIC}\\ \hline \hline \hline
 S1 & Dell PowerEdge R740 & Intel Xeon-G 6240 & - & ConnectX-5 (25 GbE) \\ %MAC
 S2 & Dell PowerEdge R740 & Intel Xeon-G 6240 & NVIDIA A2 & ConnectX-5 (25 GbE) \\ %Cheese
 S3 & Dell PowerEdge R750 & Intel Xeon-G 6330 & - & ConnectX-5 (25 GbE) \\ %Bagel
 \hline \hline
\end{tabular}%
}
\end{table}

==> tables/testbeds.tex <==
\begin{table}[t]
\centering
\caption{Testbeds}
\label{tab:testbeds}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{||c|c|c||}
    \hline \hline
    \textbf{Name} & \textbf{Machines} & \textbf{Network} \\ \hline \hline \hline
    \texttt{Direct Connection} & M1 $\leftrightarrow$ M2 & 25Gbps  \\
    \texttt{Mulit-level Connection} & M1  $\leftrightarrow$ M2 $\leftrightarrow$ M3 & 25Gbps  \\
    \hline \hline
\end{tabular}%
}
\writingtodo{Change this with a large topology graph}
\end{table}

